Sequential Auctions of Identical Items with Budget-Constrained Bidders

In this paper, we study sequential auctions with two budget constrained bidders and any number of identical items. All prior results on such auctions consider only two items. We construct a canonical outcome of the auction that is the only natural equilibrium and is unique under a refinement of subgame perfect equilibria. We show certain interesting properties of this equilibrium; for instance, we show that the prices decrease as the auction progresses. This phenomenon has been observed in many experiments and previous theoretic work attributed it to features such as uncertainty in the supply or risk averse bidders. We show that such features are not needed for this phenomenon and that it arises purely from the most essential features: budget constraints and the sequential nature of the auction. A little surprisingly we also show that in this equilibrium one agent wins all his items in the beginning and then the other agent wins the rest. The major difficulty in analyzing such sequential auctions has been in understanding how the selling prices of the first few rounds affect the utilities of the agents in the later rounds. We tackle this difficulty by identifying certain key properties of the auction and the proof is via a joint induction on all of them.

==> difficulties.tex <==
\subsection{Difficulties} 



In particular, note that the nature of this payment-based externality
is quite different from an allocation-based externality.  Consider
trying to analyze the first round of our sequential auction.  When
dealing with allocation-based externalities, we can see that the main
outcomes an agent needs to try and identify preferences between is who
wins the item?  Unlike this (possibly large, but still) finite set of
outcomes to weigh, in our setting it is not clear what options an
agent might consider in the first round, in the following sense.  When
choosing a bid, the agent both affects whether or not the win the
object, but also how much some budget (her own, or some other agent's)
will be reduced in the next round.  Until we can understand an agent's
utility from later rounds, and how it depends on remaining budgets, we
cannot hope to understand what sorts our possible future budgets the
agent is considering, and choosing between.  Recall the earlier
example which showed that, in fact, in some settings we may not be
able to simply argue that they have a simple, monotone preference
order over these outcomes.

 
   Our best hope seems to be trying to understand how
an agent considers choosing between bids in each round, and prove
structural properties about that.

To that end, consider fixing a payment $p$ in the current round, and
considering this tradeoff; agent $1$'s preference for winning rather
than losing at a price of $p$ when there are $k$ items left is given
by
\begin{equation*}
  \left(v_1-p + u(b_1-p,b_2,k-1)\right)-u(b_1,b_2-p,k-1).
\end{equation*}
One initial hope might be that we can somehow argue that this quantity
is monotone nonincreasing in $p$; such a situation would imply we
could hope to characterize each agent's behavior via some ``maximum
acceptable price,'' with a properly chosen single-item auction.  Note,
however, that it is unclear how to prove such a thing, or even that it
is true.  Consider what this would imply about the derivative:
\begin{equation*}
  \frac{d}{dp}\left(v_1-p + u(b_1-p,b_2,k-1)-u(b_1,b_2-p,k-1)\right)
  =-1+\frac{d}{dp}u(b_1-p,b_2,k-1)-\frac{d}{dp}u(b_1,b_2-p,k-1)\le0.
\end{equation*}
Note that even if we were to assume that $u$ is increasing in $b_1$
and decreasing in $b_2$, this wouldn't be sufficient to ensure the
above property -- while we would know that the first and second terms
contribute towads satisfying this goal, the third works against it,
and so we need to understand the tradeoff.  In particular, this
assumption alone only tells us how to relate $u(b_1-p,b_2,k)$ and
$u(b_1,b_2-p,k)$ individually to $u(b_1,b_2,k)$, but not how to relate
them to each other.  Thus, to understand this expression (which is at
the heart of an agent's decision making process) we need non-trivial
understanding of the structure of these utility functions.

